Kraken: An Efficient Engine with a Uniform Dataflow for Deep Neural Networks

Deep neural networks (DNNs) have been successfully employed in a multitude of applications with remarkable performance. As such performance is achieved at a significant computational cost, several embedded applications demand fast and efficient hardware accelerators for DNNs. Previously proposed application specific integrated circuit (ASIC) architectures strive to utilize arrays of hundreds of processing elements (PEs) and reduce power-hungry DRAM accesses using multiple dataflows requiring complex PE architectures. These consume significant area and reduce the maximum clock frequency. This paper introduces the Kraken architecture, which optimally processes the convolutional layers, fully-connected layers, and matrix products of any DNN through a hardware-friendly uniform dataflow. This enables maximal data reuse of weights, inputs, and outputs, with a bare-bones PE design and on-the-fly dynamic reconfiguration. Kraken, implemented in 65-nm CMOS technology at 400 MHz, packs 672 PEs in 7.3 mm2, with a peak performance of 537.6 Gops. Kraken processes the convolutional layers of AlexNet, VGG-16, and ResNet-50 at 336.6, 17.5, and 64.2 frames/s, respectively, hence outperforming the state-of-the-art ASIC architectures in terms of overall performance efficiency, DRAM accesses, arithmetic intensity, and throughput, with 5.8x more Gops/mm2 and 1.6x more Gops/W.

==> tex/z_unused.tex <==


\begin{comment}
  - Accelerator Design
    - PEs, utilz, efficiency, power, bandwidth
  - Dataflow
    - Loop nests, Reuse distance, stationaryness, examples, tiling
, where the dimensions are the height ($H$), width ($W$) and the number of input channels ($C_i$)
\end{comment}


The key objectives of designing an accelerator for neural network inference are: increasing the inference speed, decreasing the power consumption and reducing the chip area. The energy consumption is significantly dominated by data movement than actual computation. In 45 nm process, a DRAM read and an SRAM read operation consume $695 \times$ and $5.43 \times$ more energy than a fixed-point MAC operation \cite{dnn_book}. The chip area (ASIC) or logic utilization (FPGAs) depends on number of PEs, on-chip memory and any extra control logic and is another factor that affects power consumption and cost of realization.

\subsection{Dataflow}

Storing and reading pixels and kernel arrays in their original shapes is not optimal as the data required for / resulting from successive MAC operations are stored far apart. To exploit data reuse and hence reduce DRAM accesses and associated power, the multiple dimensions of input / output pixels and kernel can be \textit{tiled} and \textit{transposed}. Tiling refers to splitting dimensions and high-dimensional transpose refers to the reordering of dimensions. The orchestration of such tiled and transposed input pixels \& weights into, and the partial sums / output pixels out of an accelerator is called \textit{dataflow}.

The design of dataflow depends on the architecture of the accelerator and the supported layer types. The goal is to exploit both temporal and spatial reuse of data. \textit{Temporal reuse} occurs when same data is used by more than once by the same PE and its \textit{reuse distance} is the number of data accesses between the access of same data. If the temporal reuse distance is less than the on-chip memory capacity, temporal reuse can be exploited by holding data on-chip between reuse, reducing energy and latency, increasing $u_t$. \textit{Spatial reuse} occurs when same data is used by multiple PEs in the same time and its reuse distance is the maximum number of data accesses between any pair of consumers that use the same data. 

Since the MAC operations of eq:\ref{eq:conv} can be performed in any order to obtain identical output, the design space for dataflows is large. A dataflow is hence formally defined by a \textit{loop nest} where the order of loops dictate temporal and spatial reuse distances. Minimizing the reuse distance of one data type (input/weights/output) often comes at the cost of increasing the reuse distance of other types. Therefore, dataflows of accelerators and their corresponding architectures are classified according to the data type whose reuse they prioritize. The outermost for loop(s) correspond to the datatype that is held \textit{stationary} to exploit its temporal / spatial reuse. 

Weight-stationary dataflows such as NVDLA \cite{nvdla}, TPU \cite{tpu}, neuFlow \cite{neuflow}, Sankaradas et al. \cite{sankaradas}, Park et al. \cite{park}, Chakradhar et al. \cite{chakradhar}, Sriram et al. \cite{sriram} and Origami \cite{origami} hold the weights in register files inside PEs over multiple operations. \textit{Input-stationary} designs such as CNN \cite{scnn} hold input pixels inside PEs while changing weights. \textit{Output-stationary} dataflows such as DaDianNao \cite{dadiannao}, DianNao \cite{diannao}, Zhang et al. \cite{zhang}, Moons et al. \cite{moons}, ShiDianNao \cite{shidiannao}, Gupta et al. \cite{gupta}, Peeman et al. \cite{peeman} are designed to minimize energy consumption of reading and writing partial sums. \textit{Row-stationary} dataflows of Eyeriss v1 \cite{eyeriss} and v2 \cite{eyeriss_v2} are designed to use register files inside PEs to maximize reuse of all weights, inputs and partial sums. 
 
\subsection{Prior Work}

Almost all DNN accelerators arrange their PEs in a 2D array of $R$ rows and $C$ columns. However they widely differ in tiling, dataflow, PE architecture and inter-communication between PEs. NVDLA \cite{nvdla} keeps weights stationary inside the PEs, such that each row computes a $c_i$ and each column computes a $c_o$. The products are shifted along the columns to accumulate $C_i$. Since $C_i$ input channels cannot fit in $R$ rows, partial sums (which are wider than inputs) need to be stored outside the engine, increasing data movement. NeuFlow \cite{neuflow}, another weight-stationary architecture ---

ShiDianNao \cite{shidiannao} keeps an output sum inside each PEs, sends a $R$ rows \& $C$ columns of input pixels and broadcasts the same $k$ to all PEs. Each PE computes a partial sum, store it in FIFOs and sends it to neighbouring PEs in consecutive clocks to be accumulated into a full spatial sum. Each PE having a FIFO requires significant on-chip distributed memory and each PE having to choose values from several nearby PEs result in large multiplexers per PE. Also, a PE is built to be able to perform addition (for average pooling) and comparison (for max pooling), which complicates PE design requiring more area. 

Eyeriss \cite{eyeriss} \cite{eyeriss_v2} introduces a new dataflow: \textit{row-stationary}. Each PE computes $K_W$ partial sums and accumulates them to perform horizontal convolution. Each PE row computes $K_H$ partial sums, shifts them along the columns to compute a row of output pixels. Hence, each of their 168 PEs has 41 word buffers and a 224 word SRAM with a word being 16 bit wide, and dedicated NOCs are used to assign work to PEs and orchestrate the RS dataflow. After each layer, the chip is paused and is reconfigured by a 1794-bit (v1) / 2134-bit (v2) command, which takes about $100\mu s$ (v1). In contrast, each of Kraken's PEs have just one register and an accumulator, reducing chip area and power significantly. The convolution engine is reconfigured on-the-go using a header of just 8-bits passed through the data stream, hence reconfiguring the pipeline in a single clock cycle, allowing back-to-back processing of layers through the pipeline. The entire orchestration of dataflow and work allocation is performed in a decentralized manner using tiny lookup tables in each core (PE column) that simply mask the tvalid and tkeep signals of the outputs to route the data.


